Human-machine Symbiosis: A Multivariate Perspective for Physically Coupled Human-machine Systems

The notion of symbiosis has been increasingly mentioned in research on physically coupled human-machine systems. Yet, a uniform specification on which aspects constitute human-machine symbiosis is missing. By combining the expertise of different disciplines, we elaborate on a multivariate perspective of symbiosis as the highest form of physically coupled human-machine systems. Four dimensions are considered: Task, interaction, performance, and experience. First, human and machine work together to accomplish a common task conceptualized on both a decision and an action level (task dimension). Second, each partner possesses an internal representation of own as well as the other partner's intentions and influence on the environment. This alignment, which is the core of the interaction, constitutes the symbiotic understanding between both partners, being the basis of a joint, highly coordinated and effective action (interaction dimension). Third, the symbiotic interaction leads to synergetic effects regarding the intention recognition and complementary strengths of the partners, resulting in a higher overall performance (performance dimension). Fourth, symbiotic systems specifically change the user's experiences, like flow, acceptance, sense of agency, and embodiment (experience dimension). This multivariate perspective is flexible and generic and is also applicable in diverse human-machine scenarios, helping to bridge barriers between different disciplines.

==> figures/HMS_Layer_Model.tex <==
\tikzset{
	block/.style = {
	rectangle,
	draw = KITgreen,
	minimum width = 10em,
	minimum height = 2em
	},	
	environ/.style = {
	chamfered rectangle,
	chamfered rectangle xsep = 1cm,
	draw = KITgreen,
	minimum width = 10em,
	minimum height = 2em
	},
	knoten/.style = {
	circle,
	draw,
	inner sep = 0mm,
	fill
	}
}

\begin{tikzpicture}

\node[block](decisionlevel) {Decision Level};
\node[block, below= of decisionlevel](actionlevel){Action Level};
\node[environ, below= of actionlevel](env){Environment};
\node[knoten, right= 0.475 of actionlevel](knot1){};

\path [->]
	(decisionlevel) edge (actionlevel)
	(actionlevel) edge (env);
	
\draw[->] (env.east) -- ++(0.5,0) |- (decisionlevel);
\draw[->] (env.east) -- ++(0.5,0) |- (actionlevel);


\end{tikzpicture}

==> figures/denscontroltikz.tex <==
% Drawing control block diagrams with tikz
%
% Simon Densborn, 2013
% simon.densborn@KA-RaceIng.de
%
% Dieses Programm ist freie Software. Sie können es unter den Bedingungen der
% GNU General Public License, wie von der Free Software Foundation
% veröffentlicht, weitergeben und/oder modifizieren, entweder gemäß Version 3
% der Lizenz oder jeder späteren Version.
%
% Die Veröffentlichung dieses Programms erfolgt in der Hoffnung, daß es Ihnen
% von Nutzen sein wird, aber OHNE IRGENDEINE GARANTIE, sogar ohne die implizite
% Garantie der MARKTREIFE oder der VERWENDBARKEIT FÜR EINEN BESTIMMTEN ZWECK.
% Details finden Sie in der GNU General Public License.
%
% Sie sollten ein Exemplar der GNU General Public License zusammen mit diesem
% Programm erhalten haben. Falls nicht, siehe <http://www.gnu.org/licenses/>. 

%
% For best results use "[thick,>=latex']" in the enviromental declaration
%
%
% Example for a block diagram:
% \begin{tikzpicture}[thick,>=latex']
%	\input{./tikz/densflowtikz}
%   	
%   % Place nodes
%	\coordinate (input);
%	\ptglied[right of=input](pt);
%	\sum[right of=pt](sum);
%	\pglied[right of=sum](p);
%	\iglied[right of=p] (i);
%	\pttglied[above of=p] (fb_p);
%	\coordinate[right of=i] (split);
%	\coordinate[right of=split] (output);
%
%   % Draw arrows
%	\draw[->] (input) node[anchor=south] {$\alpha$} -- (pt);
%	\draw[->] (pt) -- (sum);
%	\draw[->] (sum) node[anchor=south west] {$-$} -- (p);
%	\draw[->] (p) -- (i);
%	\draw     (i) -- (split);
%	\draw[->] (split) -- (output) node[anchor=south] {$\omega_{Motor}$};
%	\draw[->] (split) |- (fb_p);
%	\draw[->] (fb_p) -| (sum);
%
%   % Add factors and time constants
%	\factor(pt){K};
%	\timeconst(pt){$\tau$};
% \end{tikzpicture}

% constants to change size or style
\def\nodedist{2cm}	% minimum distance of nodes
\def\width{1.5cm}	% minimum width of block in general
\def\height{0.85cm} % minimum height of block in general
\def\iwidth{1.2cm}	% width of integrator block
	
% styles	
\tikzstyle{sum}   = [ node distance=\nodedist, draw, circle]
\tikzstyle{block} = [ node distance=\nodedist, draw, rectangle,%
					  minimum height=\height, minimum width=\width*1.5]
\tikzstyle{int}   = [ node distance=\nodedist, draw, rectangle,%
					  minimum height=\height, minimum width=\iwidth]

% TeX defines for easy placement of control blocks

% Places a node with options "#1" and position "#2" in a shape of a circle
\def\sum#1(#2)%
{%
	\node[sum]#1 (#2) {}%
};

% Places an integrator block with options "#1" at position "#2"
\def\iglied#1(#2)%
{%
	\node[int]#1 (#2) {};%
	\draw (#2) +(-\iwidth/2 ,-\height/2)  [thin]  -- +(\iwidth/2 ,\height/2)%
}

% Places an proportional block with options "#1" at position "#2"
\def\pglied#1(#2)%
{%
	\node[block]#1 (#2) {};%
	\draw (#2) +(-\width/2, \height/4) [thin] -- +(\width/2,\height/4)%
}

% Places an differential block with options "#1" at position "#2"
\def\dglied#1(#2)%
{%
	\node[block]#1 (#2) {};%
	\draw (#2) +(-\width/4, \height/2) [thin] -- %
	           +(-\width/4, -\height/4) [thin] -- +(\width/2,-\height/4)%
}

% Places an time shift block with options "#1" at position "#2"
\def\totzeitglied#1(#2)%
{%
	\node[block]#1 (#2) {};%
	\draw (#2) +(-\width/4, -\height/2) [thin] -- %
	           +(-\width/4, \height/4) [thin] -- +(\width/2,\height/4)%
}

% Places an pt1 block with options "#1" at position "#2"
\def\ptglied#1(#2)%
{%
	\node[block]#1 (#2) {};%
	\draw [shift=(#2),yshift=\height/-2 ,xshift=\width/-2,thin] %
			plot[domain=0:3] ({\x /3*\width},{(1-exp(-\x*1.8)) / (1-exp(-3*1.8)) *3/4*\height}) %
}
	
% Places an pt2 block with options "#1" at position "#2"
\def\pttglied#1(#2)%
{%
	\node[block]#1 (#2) {};%
	\draw [shift=(#2),yshift=\height/-2 ,xshift=\width/-2,thin] %
			plot[samples=50,domain=0:3] ({\x/3*\width},{3/4*\height * (1 - cos(\x * 230) * exp(-1.8*\x)) / (1 - cos(3 * 230) * exp(-1.8*3)) }) %
}	

% Places an nonlinear block with options "#1" text "#3" at position "#2"}
\def\nonlin#1(#2)#3%
{%
	\node[int,double]#1 (#2) {#3} %
}	
	
% Places a factor "#2" above block "#1"
\def \factor(#1)#2%
{%
	\draw (#1) ++(-\width/2,\height/2) node [anchor=south west] {#2} %
}

% Places a time constant "#2" above block "#1"
\def \timeconst(#1)#2%
{%
	\draw (#1) ++(\width/2,\height/2) node [anchor=south east] {#2} %
}
